Oja's Algorithm for Streaming Sparse PCA

Oja's algorithm for Streaming Principal Component Analysis (PCA) for $n$ data-points in a $d$ dimensional space achieves the same sin-squared error $O(r_{\mathsf{eff}}/n)$ as the offline algorithm in $O(d)$ space and $O(nd)$ time and a single pass through the datapoints. Here $r_{\mathsf{eff}}$ is the effective rank (ratio of the trace and the principal eigenvalue of the population covariance matrix $\Sigma$). Under this computational budget, we consider the problem of sparse PCA, where the principal eigenvector of $\Sigma$ is $s$-sparse, and $r_{\mathsf{eff}}$ can be large. In this setting, to our knowledge, \textit{there are no known single-pass algorithms} that achieve the minimax error bound in $O(d)$ space and $O(nd)$ time without either requiring strong initialization conditions or assuming further structure (e.g., spiked) of the covariance matrix. We show that a simple single-pass procedure that thresholds the output of Oja's algorithm (the Oja vector) can achieve the minimax error bound under some regularity conditions in $O(d)$ space and $O(nd)$ time. We present a nontrivial and novel analysis of the entries of the unnormalized Oja vector, which involves the projection of a product of independent random matrices on a random initial vector. This is completely different from previous analyses of Oja's algorithm and matrix products, which have been done when the $r_{\mathsf{eff}}$ is bounded.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and precede the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%



==> entrywise_concentration.tex <==
\section{Entrywise Concentration of Oja Vector}
\label{sec:entrywise_concentration_oja_vector}
In this section, we describe our results for entrywise concentration results for the estimated eigenvector, $\hatv$, obtained from Oja's algorithm, given as 
\ba{
    \hatv := \frac{B_{n}z}{\norm{B_{n}z}} \label{eq:v_hat_definition}
}
for $z \sim \mathcal{N}\bb{0,I}$ and $B_{n}$ defined in Eq~\ref{definition:Bn}. Let $\exists \eta \geq 0$ such that, 
\ba{
    \leq \eta \leq \frac{1}{4 L^{4}\sigma^{4}}\frac{\lambda_{1}-\lambda_{2}}{\lambda_{2}\Tr\bb{\Sigma}} \label{eq:learning_rate_assumption_entrywise_bounds}
}
Then, using Lemma~\ref{lemma:second_moment_recursion_with_lambda2}  with $U = e_{i}$, we have
\ba{
    \E{v_{1}^{T}B_{n}e_{i}e_{i}^{T}B_{n}^{T}v_{1}} &\leq \bbb{v_{1}\bb{i}^{2} + \frac{4\eta\lambda_{1}}{\lambda_{1}-\lambda_{2}}\Sigma_{ii}}\lone^{n} \label{eq:entrywise_general_simplified_v1}
}
and similarly, using Lemma~\ref{lemma:second_moment_recursions} we have, 
\ba{
    \E{\Tr\bb{\vp^{T}B_{n}e_{i}e_{i}^{T}B_{n}^{T}\vp}} &\leq \ltwo ^{n} + \bbb{\frac{4\eta\lambda_{1}}{\lambda_{1}-\lambda_{2}}\bb{v_{1}\bb{i}^{2}\Tr\bb{\Sigma} + 4\eta\lambda_{2}\frac{L^{4}\sigma^{4}\Tr\bb{\Sigma}}{\lambda_{1}-\lambda_{2}}}}\lone ^{n} \label{eq:entrywise_general_simplified_vp}
}
where $\Sigma_{ii} = e_{i}^{\top}\Sigma e_{i}$ denotes the $i^{\text{th}}$ diagonal element of $\Sigma$ and
\ba{
    \lone = 1 + 2\eta\lambda_{1} + 8L^{4}\sigma^{4} \eta^{2}\lambda_{1}^{2}, \;\; \ltwo =  1 + 2\eta\lambda_{2} + 4L^{4}\sigma^{4}\eta^{2}\bb{\lambda_{1}^{2} + \lambda_{2}\Tr\bb{\Sigma}} \label{eq:gamma_1_gamma_2_def}
}
These moment bounds translate to the following concentration result on the entries of $\hatv$,
\begin{restatable}[Entrywise Concentration of the Oja Vector]{lemma}{entrywiseoja} Let $\eta$ satisfy \eqref{eq:learning_rate_assumption_entrywise_bounds} and $\eta d \leq \frac{1}{\lambda_{1}}$. Then, 
\bas{
    \mathbb{P}\bb{\norm{\hatv - v_{1}}_{\infty} \geq t_{1}\norm{v_{1}}_{\infty}} \leq d_{n}
}
where for any $v \in \R^{d}$, $\norm{v}_{\infty} = \max_{i \in [d]}\left|v\bb{i}\right|$ and absolute constant $t_{1} > 0$.
\end{restatable}
\begin{proof} We start by using the definition of $\hatv$ in Eq~\ref{eq:v_hat_definition}. Therefore,
\ba{
    \mathbb{P}\bb{\norm{\hatv - v_{1}}_{\infty} \geq t_{1}\norm{v_{1}}_{\infty}} &= \mathbb{P}\bb{\max_{i \in [d]}\left|\hatv\bb{i} - v_{1}\bb{i}\right| \geq t_{1}\norm{v_{1}}_{\infty}} \notag \\
    &= \mathbb{P}\bb{\max_{i \in [d]}\left|\frac{e_{i}^{\top}B_{n}z}{\norm{B_{n}z}} - v_{1}\bb{i}\right| \geq t_{1}\norm{v_{1}}_{\infty}} \notag \\
    &= \mathbb{P}\bb{\max_{i \in [d]}\left|\bb{\frac{e_{i}^{\top}B_{n}z}{\lone^{\frac{n}{2}}} - v_{1}\bb{i}} + e_{i}^{\top}B_{n}z\bb{\frac{1}{\norm{B_{n}z}} - \frac{1}{\lone^{\frac{n}{2}}}}\right| \geq t_{1}\norm{v_{1}}_{\infty}} \notag \\
    &\leq \mathbb{P}\bb{\max_{i \in [d]}\left|\frac{e_{i}^{\top}B_{n}z}{\lone^{\frac{n}{2}}} - v_{1}\bb{i}\right| \geq \frac{1}{2}t_{1}\norm{v_{1}}_{\infty}} \notag \\
    & \;\;\;\; + \mathbb{P}\bb{\max_{i \in [d]}\left|e_{i}^{\top}B_{n}z\bb{\frac{1}{\norm{B_{n}z}} - \frac{1}{\lone^{\frac{n}{2}}}}\right| \geq \frac{1}{2}t_{1}\norm{v_{1}}_{\infty}}
}
Define the events 
\bas{
    \mathcal{E}_{1} := \max_{i \in [d]}\left|\frac{e_{i}^{\top}B_{n}z}{\lone^{\frac{n}{2}}} - v_{1}\bb{i}\right| \geq \frac{1}{2}t_{1}\norm{v_{1}}_{\infty}, \;\;\; \mathcal{E}_{2} := \max_{i \in [d]}\left|e_{i}^{\top}B_{n}z\bb{\frac{1}{\norm{B_{n}z}} - \frac{1}{\lone^{\frac{n}{2}}}}\right| \geq \frac{1}{2}t_{1}\norm{v_{1}}_{\infty}
}
Let $r_{i} := e_{i}^{\top}B_{n}z$. We start with $\mathcal{E}_{1}$,
\bas{
    \mathbb{P}\bb{\mathcal{E}_{1}} &\leq \sum_{i \in [d]}\mathbb{P}\bb{\left|\frac{e_{i}^{\top}B_{n}z}{\lone^{\frac{n}{2}}} - v_{1}\bb{i}\right| \geq \frac{1}{2}t_{1}\norm{v_{1}}_{\infty}} \\
    &= \sum_{i \in [d]}\mathbb{P}\bb{\left|r_{i} - v_{1}\bb{i}\lone^{\frac{n}{2}}\right| \geq \frac{1}{2}t_{1}\lone^{\frac{n}{2}}\norm{v_{1}}_{\infty}} \\
    &\leq 4\sum_{i \in [d]}\frac{\mathbb{E}\bbb{\bb{r_{i} - v_{1}\bb{i}\lone^{\frac{n}{2}}}^{2}}}{t_{1}^{2}\lone^{n}\norm{v_{1}}_{\infty}^{2}} \\
    &= \frac{4}{t_{1}^{2}}\sum_{i \in [d]}\frac{\mathbb{E}\bbb{r_{i}^{2}} - v_{1}\bb{i}^{2}\lone^{n}}{\norm{v_{1}}_{\infty}^{2}\lone^{n}} \\
    &= \frac{4}{t_{1}^{2}}\sum_{i \in [d]}\frac{\mathbb{E}\bbb{e_{i}^{\top}B_{n}zz^{\top}B_{n}^{\top}e_{i}} - v_{1}\bb{i}^{2}\lone^{n}}{\norm{v_{1}}_{\infty}^{2}\lone^{n}} \\
    &= \frac{4}{t_{1}^{2}}\sum_{i \in [d]}\frac{\mathbb{E}\bbb{e_{i}^{\top}B_{n}v_{1}v_{1}^{\top}B_{n}^{\top}e_{i}} + \mathbb{E}\bbb{e_{i}^{\top}B_{n}\vp\vp^{\top}B_{n}^{\top}e_{i}} - v_{1}\bb{i}^{2}\lone^{n}}{\norm{v_{1}}_{\infty}^{2}\lone^{n}} \\
    &\leq \frac{4}{t_{1}^{2}}\sum_{i \in [d]}\frac{\frac{4\eta\lambda_{1}\Sigma_{ii}}{\lambda_{1}-\lambda_{2}}\lone^{n} + \ltwo ^{n} + \bbb{\frac{4\eta\lambda_{1}}{\lambda_{1}-\lambda_{2}}\bb{v_{1}\bb{i}^{2}\Tr\bb{\Sigma} + 4\eta\lambda_{2}\frac{L^{4}\sigma^{4}\Tr\bb{\Sigma}}{\lambda_{1}-\lambda_{2}}}}\lone ^{n}}{\norm{v_{1}}_{\infty}^{2}\lone^{n}}, \text{ using Eq}~\ref{eq:entrywise_general_simplified_v1}, ~\ref{eq:entrywise_general_simplified_vp} \\
    &= \frac{4}{\norm{v_{1}}_{\infty}^{2}t_{1}^{2}}\bb{\frac{8\eta\lambda_{1}\Tr\bb{\Sigma}}{\lambda_{1}-\lambda_{2}} + d\frac{\ltwo^{n}}{\lone^{n}} + 16L^{4}\sigma^{4}\Tr\bb{\Sigma}\frac{d\eta^{2}\lambda_{1}\lambda_{2}}{\bb{\lambda_{1}-\lambda_{2}}^{2}} }
}

\end{proof}



==> original_writeup_joint_sparse_pca.tex <==
\subsection{\rd Original Writeup [This Section is to be removed] \bk}

Our method is described in Algorithm~\ref{alg:cardinality_support}. It takes as input the dataset $\left\{X_{i}\right\}_{i \in [n]}$, the learning rate $\eta$ and a truncation parameter $k$, which denotes the desired sparsity level. When given a dataset $\left\{X_{i}\right\}_{i \in [n]}$, we split the dataset into two parts of equal size. Using the first half set of samples, we estimate the support set $\widehat{S}$, and using the second half of samples we estimate $v_{1}$. Both procedures use Oja's Algorithm as a subroutine. We analyze two natural ideas for support recovery - A cardinality-based truncation method in Algorithm~\ref{alg:cardinality_support}, and a value-based truncation method in Algorithm~\ref{alg:threshold_support} (Section~\ref{section:alternate_truncation} of the Appendix).
%\begin{minipage}{0.46\textwidth}
  \begin{algorithm}[H]
\caption{$\CardinalitySupport\bb{\left\{X_{i}\right\}_{i \in [n]}, k, \eta}$} \label{alg:cardinality_support}
\begin{algorithmic}[1]
\STATE \textbf{Input} : Dataset $\left\{X_{i}\right\}_{i \in [n]}$, learning rate $\eta > 0$, Cardinality parameter $k \geq s$
\STATE $w_{0}, y_{0} \sim \mathcal{N}\bb{0,I}$
\STATE $\hat{v}_1\leftarrow \SparsePCA\bb{\left\{X_{i}\right\}_{i \in [n/2]}, \eta, y_{0}}$
\STATE $\hat{v}_2\leftarrow \SparsePCA\bb{\left\{X_{i}\right\}_{i \in \{n/2+1,\dots,n\}}, \eta, w_{0}}$
\STATE $\widehat{S} \leftarrow \text{ Indices of } k \text{ largest values of} \left|\hat{v}_1\right|$
%\STATE $\widehat{v} \leftarrow \lfloor\hat{v}_2\rfloor_{\hatS}$
\STATE $\vojatopk \leftarrow \frac{\trunc{\widehat{v}_2}{\widehat{S}}}{\norm{\trunc{\widehat{v}_2}{\widehat{S}}}_{2}}$
\RETURN $\bbb{\vojatopk, \widehat{S}}$
\end{algorithmic}
\end{algorithm} 
%    \begin{algorithm}[H]
% \caption{$\CardinalitySupport\bb{\left\{X_{i}\right\}_{i \in [n]}, k, \eta}$} \label{alg:cardinality_support}
% \begin{algorithmic}[1]
% \STATE \textbf{Input} : Dataset $\left\{X_{i}\right\}_{i \in [n]}$, learning rate $\eta > 0$, Cardinality parameter $k \geq s$
% \STATE Set $i \leftarrow 0$ and choose $y_0 \sim \mathcal{N}\bb{0,I}$
% \FOR{t in range[1, $n$]}
% \STATE $i \leftarrow i + 1$
% \STATE $y_{i} \leftarrow (I + \eta X_{t}X_{t}^{T})y_{i-1}, \;\; y_{i} \leftarrow \frac{y_{i}}{\|y_{i}\|_{2}}$
% \ENDFOR
% \STATE $\widehat{S} \leftarrow \text{ Set of largest } k \text{ indices, in absolute value, of } y_{i}$
% \STATE $\widehat{v} \leftarrow \SparsePCA\bb{\left\{X_{i}\right\}_{i \in [n]}, \eta, \widehat{S}}$
% \STATE $v_{\text{oja}} \leftarrow \frac{\trunc{\widehat{v}}{\widehat{S}}}{\norm{\trunc{\widehat{v}}{\widehat{S}}}_{2}}$
% \RETURN $\bb{v_{\text{oja}}, \widehat{S}}$
% \end{algorithmic}
% \end{algorithm} 
%\end{minipage}
% \begin{minipage}{0.47\textwidth}
%   \begin{algorithm}[H]
% \caption{$\CardinalitySupport\bb{\left\{X_{i}\right\}_{i \in [n]}, k, \eta}$} \label{alg:cardinality_support}
% \begin{algorithmic}[1]
% \STATE \textbf{Input} : Dataset $\left\{X_{i}\right\}_{i \in [n]}$, learning rate $\eta > 0$, Cardinality parameter $k \geq s$
% \STATE $\hat{v}_1\leftarrow \SparsePCA\bb{\left\{X_{i}\right\}_{i \in [n/2]}, \eta}$
% \STATE $\hat{v}_2\leftarrow \SparsePCA\bb{\left\{X_{i}\right\}_{i \in \{n/2+1,\dots,n\}}, \eta}$
% \STATE $\widehat{S} \leftarrow \text{ Indices of } k \text{ largest values in maginude of } \hat{v}_1$
% \STATE $\widehat{v} \leftarrow \SparsePCA\bb{\left\{X_{i}\right\}_{i \in [n]}, \eta, \widehat{S}}$
% \STATE $v_{\text{oja}} \leftarrow \frac{\trunc{\widehat{v}}{\widehat{S}}}{\norm{\trunc{\widehat{v}}{\widehat{S}}}_{2}}$
% \RETURN $\bb{v_{\text{oja}}, \widehat{S}}$
% \end{algorithmic}
% \end{algorithm} 
% \end{minipage}
\thmrestate{Convergence of $\CardinalitySupport$}{convergencecardinalitysupport}{
    \label{theorem:convergence_cardinality_support}
    Let $\vojatopk, \;\; \hatS$ be obtained from Algorithm~\ref{alg:cardinality_support}. Set the learning rate as $\eta := \frac{3\log\bb{\effecrank}}{{n\bb{\lambda_{1}-\lambda_{2}}}}$. Then, for $n =\widetilde{\Omega}\bb{\frac{1}{\min_{i\in \sh}v_{1}\bb{i}^{2}}\frac{\lambda_{1}}{\lambda_{1}-\lambda_{2}}}^{2}$, with probability at least $3/4$, we have, for absolute constant $C'' > 0$,
    \bas{
        \sin^{2}\bb{\vojatopk, v_{1}} \leq C''\bb{\frac{\lambda_{1}}{ \lambda_{1}-\lambda_{2}}}^{2}\frac{k\log\bb{\effecrank}}{n}, \; \text{ and} \; \sh \subseteq \hatS,
    }
}
% \begin{proof}
%     Let $\mathcal{E} := \left\{\sh \subseteq \hatS \right\}$. Consider the following variables from Theorem~\ref{theorem:convergence_truncated_oja}:
%     \bas{
%         & W_{\hatS} := \E{I_{\hatS}-I_{\hatS}v_{1}v_{1}^{T}I_{\hatS}\;|\;\mathcal{E}}, \; G_{\hatS} := \E{I_{S \bigcap \hatS}\;|\;\mathcal{E}} \\ 
%         & \alpha_{0} := v_{1}^{T}W_{\hatS}v_{1}, \; \beta_{0} := \Tr\bb{\vp^{T}W_{\hatS}\vp}, \; p_{0} := v_{1}^{T}G_{\hatS}v_{1}, \; q_{0} := \Tr\bb{\vp^{T}G_{\hatS}\vp}
%     }
%     Since $|\hatS| = k$, therefore, 
%     \bas{
%         \beta_{0} = \Tr\bb{\vp^{T}W_{\hatS}\vp} \leq \Tr\bb{W_{\hatS}} \leq \Tr\bb{\hatS} = k
%     }
%     Furthermore, under event $\mathcal{E}$, $\sh \subseteq \left\{S \bigcap \hatS\right\}$. Therefore, 
%     \bas{
%         p_{0} &= v_{1}^{T}G_{\hatS}v_{1} \geq \sum_{i \in \sh}v_{1}\bb{i}^{2} = 1 - \sum_{i \notin \sh}v_{1}\bb{i}^{2} \geq 1 - \frac{s\log\bb{\effecrank}}{n}, \text{ using definition of } \sh
%     }
%     To verify the assumption on $p_{0}$ mentioned in Theorem~\ref{theorem:convergence_truncated_oja}, it is sufficient to ensure
%     \bas{
%         \eta\lambda_{1}s \bb{\frac{20\lambda_{1}}{\lambda_{1}-\lambda_{2}}} \leq \bb{1 - \frac{s\log\bb{\effecrank}}{n}}\bb{1+\frac{\delta}{4}} - 1
%     }
%     which is true by the definition on $\eta$ and $n$. Lastly, 
%     \bas{
%         \alpha_{0} &= v_{1}^{T}W_{\hatS}v_{1} = \E{v_{1}^{T}I_{\hatS}v_{1}-\bb{v_{1}^{T}I_{\hatS}v_{1}}^{2}\;|\;\mathcal{E}} \\
%                    &\leq 1 - \E{v_{1}^{T}I_{\hatS}v_{1}\;|\;\mathcal{E}}, \text{ using }  v_{1}^{T}I_{\hatS}v_{1} \leq 1 \\
%                    &\leq 1 - \sum_{i \in \sh}v_{1}\bb{i}^{2}, \text{ since } \sh \subseteq \hatS \\
%                    &= \sum_{i \notin \sh}v_{1}\bb{i}^{2} \leq \frac{s\log\bb{\effecrank}}{n} \geq \frac{1}{2}
%     }
%     Therefore, using Theorem~\ref{theorem:convergence_truncated_oja}, with probability at least $1-\delta-\mathbb{P}\bb{\mathcal{E}^{c}}$,
%     \ba{
%         \sin^{2}\bb{v_{\text{oja}}, v_{1}} \leq \frac{C'\log\bb{\frac{1}{\delta}}}{\delta^{3}}\frac{5\lambda_{1}}{\lambda_{1}-\lambda_{2}}\eta\lambda_{1}k \label{eq:cardinality_sin_squared_bound}
%     }
%     We now upper bound $\mathbb{P}\bb{\mathcal{E}^{c}}$. Define $r_{i}:= e_{i}^{T}B_{n}y_{0},$ $i \in [d]$. Observe that 
%     \bas{
%         \mathcal{E} \iff \exists \tau_{n} > 0 \text{ such that } \left\{\forall i \in \sh, |r_{i}| \geq \tau_{n}\right\} \bigcap \left\{\left|\left\{i : i \notin \sh, |r_{i}| \geq \tau_{n} \right\}\right| \leq k-s'\right\}
%     }
%     or equivalently, 
%     \bas{
%         \mathcal{E}^{c} \iff \forall \tau_{n} > 0, \left\{\exists i \in \sh, |r_{i}| \leq \tau_{n}\right\} \bigcup \left\{\left|\left\{i : i \notin \sh, |r_{i}| \geq \tau_{n} \right\}\right| > k-s'\right\}
%     }
%     Therefore, for any fixed $\tau_{n} > 0$ 
%     \bas{
%         \mathcal{E}^{c} &\implies \left\{\exists i \in \sh, |r_{i}| \leq \tau_{n}\right\} \bigcup \left\{\left|\left\{i : i \notin \sh, |r_{i}| \geq \tau_{n} \right\}\right| > k-s'\right\} \\
%         &\implies \left\{\exists i \in \sh, |r_{i}| \leq \tau_{n}\right\} \bigcup \left\{\left|\left\{i : i \notin \sh, |r_{i}| \geq \tau_{n} \right\}\right| > k-s\right\}
%     }
%     Let $\mathcal{G} := \left\{ |v_{1}^{T}y_{0}| \geq \frac{\delta}{\sqrt{e}} \right\}$ and threshold $\tau_{n}:= \frac{\delta}{\sqrt{2e}}\min_{i \in \sh}|v_{1}\bb{i}|\bb{1+\eta\lambda_{1}}^{n}$. Using a union-bound, 
%     \bas{
%         \mathbb{P}\bb{\mathcal{E}^{c}} &\leq \mathbb{P}\bb{\left\{\exists i \in \sh, |r_{i}| \leq \tau_{n}\right\}} + \mathbb{P}\bb{\left\{\left|\left\{i : i \notin \sh, |r_{i}| \geq \tau_{n} \right\}\right| > k-s\right\}} \\
%         &\leq \mathbb{P}\bb{\left\{\exists i \in \sh, |r_{i}| \leq \tau_{n}\right\}} + \frac{\sum_{i \notin \sh}\mathbb{P}\bb{|r_{i}| \geq \tau_{n}}}{k-s+1}, \text{ using Markov's inequality} \\
%         &= \mathbb{P}\bb{G}\mathbb{P}\bb{\left\{\exists i \in \sh, |r_{i}| \leq \tau_{n} \bigg| \mathcal{G}\right\}} + \mathbb{P}\bb{G}^{C}\mathbb{P}\bb{\left\{\exists i \in \sh, |r_{i}| \leq \tau_{n} \bigg| \mathcal{G}^{c}\right\}} + \\
%         & \;\;\;\; + \frac{\sum_{i \notin \sh}\mathbb{P}\bb{|r_{i}| \geq \tau_{n}}}{k-s+1} \\
%         &\leq \mathbb{P}\bb{G}^{C} + \mathbb{P}\bb{\left\{\exists i \in S, |r_{i}| \leq \tau_{n} \bigg| \mathcal{G}\right\}} + \frac{\sum_{i \notin \sh}\mathbb{P}\bb{|r_{i}| \geq \tau_{n}}}{k-s+1} \\
%         &\leq \mathbb{P}\bb{G}^{C} + \sum_{i \in \sh}\mathbb{P}\bb{|r_{i}| \leq \tau_{n}\bigg| \mathcal{G}} + \frac{\sum_{i \notin \sh}\mathbb{P}\bb{|r_{i}| \geq \tau_{n}}}{k-s+1} \\
%         &\leq \mathbb{P}\bb{G}^{C} + \underbrace{\sum_{i \in \sh}\mathbb{P}\bb{|r_{i}| \leq \tau_{n}\bigg| \mathcal{G}}}_{T_{1}} + \underbrace{\frac{\sum_{i \in S \bigcap S^{'C}}\mathbb{P}\bb{|r_{i}| \geq \tau_{n}}}{k-s+1}}_{T_{2}} + \underbrace{\frac{\sum_{i \notin S}\mathbb{P}\bb{|r_{i}| \geq \tau_{n}}}{k-s+1}}_{T_{3}}
%     }
%     For $T_{2}$, using Markov's inequality and Eq~\ref{eq:v1_i_second_moment} along with $\bb{1+x} \geq \exp\bb{x-x^{2}} \forall x \geq 0$ we have,
%     \bas{
%         \mathbb{P}\bb{|r_{i}| \geq \tau_{n}} &\leq \frac{\E{r_{i}^{2}}}{\tau_{n}^{2}}
%         \leq 10e\frac{\sum_{i \in S \bigcap S^{'C}}v_{1}\bb{i}^{2}}{\delta^{2}\min_{i \in \sh}v_{1}\bb{i}^{2}} \leq \frac{10e }{\delta^{2}\min_{i \in \sh}v_{1}\bb{i}^{2}}\frac{s\log\bb{\effecrank}}{n}
%     }
%     Using Lemma~\ref{lemma:gaussian_anti_concentration}, we have $\mathbb{P}\bb{G}^{C} \leq \delta$. We bound $T_{1}$ and $T_{3}$ using Lemmas~\ref{lemma:i_in_S_bound} and ~\ref{lemma:i_notin_S_bound} respectively. Therefore, 
%     \bas{
%         \mathbb{P}\bb{\mathcal{E}^{c}} &\leq \delta + \eta \lambda_{1}s\log\bb{\effecrank} + 24\eta\lambda_{1}\bb{\frac{4\lambda_{1}}{\bb{\lambda_{1}-\lambda_{2}}}}\sum_{i \in \sh}\frac{1}{v_{1}\bb{i}^{2}} + 12\eta^{2}\lambda_{1}^{2}\bb{\frac{4\lambda_{1}}{\bb{\lambda_{1}-\lambda_{2}}}}^{2}\sum_{i \in \sh}\frac{1}{v_{1}\bb{i}^{4}} \\
%         & \;\;\;\; + \frac{10e }{\delta^{2}\min_{i \in \sh}v_{1}\bb{i}^{2}}\frac{s\log\bb{\effecrank}}{\bb{k-s+1}n} + \bb{\frac{400e^{2}\bb{4\lambda_{1}}^{2}}{\delta^{4}\bb{k-s+1}\bb{\min_{i \in \sh}v_{i}^{4}}\bb{\lambda_{1}-\lambda_{2}}^{2}}} \eta^{2}\lambda_{1}^{2}d \\
%         &\leq 5\delta
%     }
%     where the last inequality follows by using the bound on $n$. The result then follows using Eq~\ref{eq:cardinality_sin_squared_bound} and setting $\delta$ smaller by a constant.
% \end{proof}
% \begin{theorem}
%     \label{theorem:convergence_threshold_support}
%     (Convergence of $\ThresholdSupport$) Let $\hatS$ be obtained from Algorithm~\ref{alg:threshold_support} and subsequently used in Algorithm~\ref{alg:truncated_oja}. Fix a value of $\delta \in \bb{0,1}$. Let the step-size, $\eta$ satisfy $\bb{1-\theta}\bb{\lambda_{1}-\lambda_{2}} + 25L^4\sigma^{4}\eta\lambda_{1}^{2} = 25L^4\sigma^{4}\log\bb{\effecrank}\eta\lambda_{2}\Tr\bb{\Sigma}$ for $\theta \in \bb{\frac{1}{2}, 1}$ and $\eta L^2\sigma^{2}\leq \frac{1}{4}\min\left\{\frac{1}{\lambda_{1}}, \frac{\log\bb{\effecrank}}{\Tr\bb{\Sigma}}, \frac{\log\bb{\effecrank}}{\sqrt{\lambda_{1}\Tr\bb{\Sigma}}}\right\}$. Define $\sh := \left\{i : i \in S, \; |v_{1}\bb{i}| \geq \sqrt{\frac{\log\bb{\effecrank}}{n}} \right\}, \; s' := |\sh| \leq s$ and threshold $\gamma_{n}:= \frac{\delta}{\sqrt{2e}}\min_{i \in \sh}|v_{1}\bb{i}|\bb{1+\eta\lambda_{1}}^{n}$. Then for $n \geq \bb{\frac{80e\lambda_{1}}{\delta^{2}\sqrt{s}\min_{i\in \sh}v_{1}\bb{i}^{2}\bb{\lambda_{1}-\lambda_{2}}}}^{2}$, with probability at least $1-\delta$, 
%     \bas{
%         \sin^{2}\bb{v_{\text{oja}}, v_{1}} \leq \frac{C''\log\bb{\frac{1}{\delta}}}{\delta^{3}}\frac{\lambda_{1}}{\lambda_{1}-\lambda_{2}}\frac{\max\left\{s, \log\bb{\effecrank}\right\}\log\bb{\effecrank}}{n}
%     }
%     where $C'' > 0$ is an absolute constant.
% \end{theorem}
% \begin{proof}
%     Consider the setting of Theorem~\ref{theorem:convergence_truncated_oja}. Let $\mathcal{E}$ be the event $\left\{ |v_{1}^{T}y_{0}| \geq \frac{\delta}{\sqrt{e}} \right\}$. By Lemma~\ref{lemma:gaussian_anti_concentration}, $\mathbb{P}\bb{\mathcal{E}} \geq 1-\delta$. Recall the definitions,  
%     \bas{
%         & W_{\hatS} := \E{I_{\hatS}-I_{\hatS}v_{1}v_{1}^{T}I_{\hatS} \bigg| \mathcal{E}}, \; G_{\hatS} := \E{I_{S \bigcap \hatS} \bigg| \mathcal{E}} \\ 
%         & \alpha_{0} := v_{1}^{T}W_{\hatS}v_{1}, \; \beta_{0} := \Tr\bb{\vp^{T}W_{\hatS}\vp}, \; p_{0} := v_{1}^{T}G_{\hatS}v_{1}
%     }
%     We upper bound $\alpha_{0}$, $\beta_{0}$ and lower bound $p_{0}$ under the setting of Algorithm \ref{alg:cardinality_support}. Define $r_{i} := e_{i}^{T}B_{n}y_{0}, i \in [d]$.
%     For $\alpha_{0}, p_{0}$, we have
%     \ba{
%       \alpha_{0} &= v_{1}^{T}W_{\hatS}v_{1} = \E{v_{1}^{T}I_{\hatS}v_{1} - \bb{v_{1}^{T}I_{\hatS}v_{1}}^{2}\bigg| \mathcal{E}} \notag \\
%        &= \E{v_{1}^{T}I_{\hatS}v_{1}\bb{1 - v_{1}^{T}I_{\hatS}v_{1}}\bigg| \mathcal{E}} \notag \\
%        &\leq 1 - \E{v_{1}^{T}I_{\hatS}v_{1}\bigg| \mathcal{E}}, \text{ using } v_{1}^{T}I_{\hatS}v_{1} \leq 1 \notag \\
%        &= 1 - \sum_{i \in S}v_{1}\bb{i}^{2}\mathbb{P}\bb{i \in \hatS; i \in S \bigg| \mathcal{E}}, \notag \\
%        &= \sum_{i \in S}v_{1}\bb{i}^{2}\mathbb{P}\bb{i \notin \hatS; i \in S \bigg| \mathcal{E}}\label{eq:cardinality_based_threshold_alpha0_bound}
%     }
%     \ba{
%         p_{0} &= v_{1}^{T}G_{\hatS}v_{1} \notag \\
%               &= v_{1}^{T}\E{I_{S\bigcap \hatS}}v_{1} \notag \\
%               % &= \sum_{i \in S \bigcap \hatS}v_{1}\bb{i}^{2}\mathbb{P}\bb{i \in \hatS; i\in S \bigg| \mathcal{E}} \notag \\
%               &= \sum_{i \in S}v_{1}\bb{i}^{2}\mathbb{P}\bb{ i \in \hatS; i\in S \bigg| \mathcal{E}}  \notag \\
%               &= 1 - \sum_{i \in S}v_{1}\bb{i}^{2}\mathbb{P}\bb{ i \notin \hatS ; i\in S \bigg| \mathcal{E}} \label{eq:cardinality_based_threshold_p0_bound} 
%     }
%     Therefore, for both $\alpha_{0}, p_{0}$, we seek to upper bound $\sum_{i \in S}v_{1}\bb{i}^{2}\mathbb{P}\bb{i \notin \hatS; i\in S\bigg| \mathcal{E}}$. We have
%     \bas{
%         & \sum_{i \in S}v_{1}\bb{i}^{2}\mathbb{P}\bb{i \notin \hatS; i\in S\bigg| \mathcal{E}} \\
%         &\;\;\;\;= \sum_{i \in \sh}v_{1}\bb{i}^{2}\mathbb{P}\bb{i \notin \hatS; i\in S\bigg| \mathcal{E}} + \sum_{i \in S \setminus \sh}v_{1}\bb{i}^{2}\mathbb{P}\bb{i \notin \hatS; i\in S\bigg| \mathcal{E}} \\
%         &\;\;\;\;\leq \frac{s\log\bb{\effecrank}}{n} + \sum_{i \in \sh}v_{1}\bb{i}^{2}\mathbb{P}\bb{i \notin \hatS; i\in S\bigg| \mathcal{E}} \\
%         &\;\;\;\;= \frac{s\log\bb{\effecrank}}{n} + \sum_{i \in \sh}v_{1}\bb{i}^{2}\mathbb{P}\bb{|r_{i}| < \gamma_{n} ; i \in S \bigg| \mathcal{E}} \\
%         &\;\;\;\;\stackrel{(i)}{\leq} \frac{s\log\bb{\effecrank}}{n} + \sum_{i \in \sh}v_{1}\bb{i}^{2}\bbb{\eta \lambda_{1}\log\bb{\effecrank} + 24\eta\lambda_{1}\bb{\frac{4\lambda_{1}}{\bb{\lambda_{1}-\lambda_{2}}}}\frac{1}{v_{1}\bb{i}^{2}} + 12\eta^{2}\lambda_{1}^{2}\bb{\frac{4\lambda_{1}}{\bb{\lambda_{1}-\lambda_{2}}}}^{2}\frac{1}{v_{1}\bb{i}^{4}}} \\
%         &\;\;\;\;= \frac{s\log\bb{\effecrank}}{n} + \eta \lambda_{1}\log\bb{\effecrank} + 24\eta\lambda_{1}s'\bb{\frac{4\lambda_{1}}{\bb{\lambda_{1}-\lambda_{2}}}} + 12\eta^{2}\lambda_{1}^{2}\bb{\frac{4\lambda_{1}}{\bb{\lambda_{1}-\lambda_{2}}}}^{2}\sum_{i \in \sh}\frac{1}{v_{1}\bb{i}^{2}} \\
%         &\;\;\;\;\leq 100\eta\lambda_{1}\left\{s, \log\bb{\effecrank}\right\} \leq \frac{1}{2}, \text{ using } |v_{1}\bb{i}| \geq \sqrt{\frac{\log\bb{\effecrank}}{n}}, i \in \sh
%     }
%     For $\beta_{0}$ we have
%     \bas{
%         \beta_{0} &\leq \E{\Tr\bb{W_{\hatS}}\bigg| \mathcal{E}} = \sum_{i \in [d]}\mathbb{P}\bb{i \in \hatS \bigg| \mathcal{E}} - \sum_{i \in S}v_{1}\bb{i}^{2}\mathbb{P}\bb{i \in \hatS \bigg| \mathcal{E}} \\
%         &\leq \sum_{i \notin S}\mathbb{P}\bb{i \in \hatS \bigg| \mathcal{E}} + \sum_{i \in S}\bb{1-v_{1}\bb{i}^{2}}\mathbb{P}\bb{i \in \hatS \bigg| \mathcal{E}} \\
%         &= \sum_{i \notin S}\mathbb{P}\bb{i \in \hatS \bigg| \mathcal{E}} + s-1 \\
%         &\leq \sum_{i \notin S}\mathbb{P}\bb{|r_{i}| \geq \gamma_{n}\bigg| \mathcal{E}} + s-1 \\
%         &= \sum_{i \notin S}\frac{\mathbb{P}\bb{|r_{i}| \geq \gamma_{n}}}{\mathbb{P}\bb{\mathcal{E}}} + s-1 \\
%         &\leq 2\sum_{i \notin S}\mathbb{P}\bb{|r_{i}| \geq \gamma_{n}} + s - 1, \text{ since } \mathbb{P}\bb{\mathcal{G}} \geq 1-\delta \\ 
%         &\leq \bb{\frac{800e^{2}\bb{4\lambda_{1}}^{2}}{\delta^{4}\bb{\min_{i \in S}v_{i}^{4}}\bb{\lambda_{1}-\lambda_{2}}^{2}}} \eta^{2}\lambda_{1}^{2}d + s-1, \text{ using Lemma}~\ref{lemma:i_notin_S_bound} \\
%         &\leq 2s \text{, using bound on } n
%     }
%     The result then follows using Theorem~\ref{theorem:convergence_truncated_oja} and substituting the bounds on $\alpha_{0}$, $\beta_{0}$ and $p_{0}$.
% \end{proof}
% \rd Add boosting proposition here\bk
% \rd Say how boosting helps \bk
% \rd make plot \bk
% \noindent
The error rate in Theorem~\ref{theorem:convergence_cardinality_support} is optimal in its dependence on $s, n$ and near-optimal in its dependence on $\lambda_{1}, \lambda_{2}$. We leave the improvement of the dependence on $\lambda_{1}, \lambda_{2}$ to match the corresponding lower bound in \cite{pmlr-v22-vu12, cai2013sparse} for future work.
Note that a constant probability result can be boosted to a high probability one using multiple independent runs and performing geometric aggregation. Formally, see Lemma~\ref{lemma:sin2_geometric_aggregation}, which follows due to Claim 1 from ~\cite{kelner2023semi}. The proof is included in Appendix Section~\ref{appendix:useful_results}.
\lemmarestate{Geometric Aggregation for Boosting}{sin2geometricaggregation}{
    \label{lemma:sin2_geometric_aggregation}
    Let $u_{*} \in \mathbb{R}^{d}$ be a fixed unit vector and $\left\{u_{i}\right\}_{i \in [n]}$, $u_{i} \in \R$ be $r$ independent random unit vectors each satisfying $\mathbb{P}\bb{\sin^{2}\bb{u_{i},u_{*}} \geq \epsilon} \leq p$ for a constant $p \in \bb{0,\frac{1}{2}}$. There there is an estimator $\tilde{u}$ which selects one of $\left\{u_{i}\right\}_{i \in [r]}$, runs in $O\bb{r^{2}d}$ time and satisfies $ \mathbb{P}\bb{\sin^{2}\bb{\tilde{u}, u_{*}} \geq 9\epsilon} \leq \exp\bb{-\frac{\bb{1-p}r}{20}}$.
}
Therefore, inflating the sample complexity by $O\bb{\log\bb{\frac{1}{\delta}}}$, we can obtain a success probability of atleast $1-\delta$ for any $\delta > 0$ at a cost of an additive $O\bb{d\log^{2}\bb{\frac{1}{\delta}}}$ increase in the overall runtime.

\begin{remark}
    Consider $\forall i \in S, \; v_{1}\bb{i} = \frac{1}{\sqrt{s}}$. Then, the bound provided in Theorem~\ref{theorem:convergence_cardinality_support} requires $n = \widetilde{\Omega}\bb{s^{2}}$, which is necessary for guarantees provided in some contemporary work on Sparse PCA and support recovery such as ~\cite{meinshausen2006high, bresler2018sparse, qiu2019gradientbased} and Proposition 1 in ~\cite{amini2008high}. In comparison, other algorithms such as ~\cite{pmlr-v37-yangd15, yuan2011truncated} and Proposition 2 in ~\cite{amini2008high} require $n = \widetilde{\Omega}\bb{s}$ and either use SDP-based relaxations or require a stronger initialization condition. Based on experimental results, we believe that this is an artifact of our moment-based analysis and can be relaxed to $n = \widetilde{\Omega}\bb{s}$ with more sophisticated concentration inequalities.
    % The guarantees proven in Theorem~\ref{theorem:convergence_cardinality_support} are meaningful only when $n =\widetilde{\Omega} \bb{\frac{1}{\min_{i\in \sh}v_{1}\bb{i}^{4}}}$. From Assumption~\ref{assumption:high_dimensions}, we have $\frac{d}{n} = \dnratio$ for an absolute constant $\dnratio$. Combining the two, this implies that the valid parameter regime for Theorem~\ref{theorem:convergence_cardinality_support} is $\min_{i\in \sh}|v_{1}\bb{i}| \geq \Omega\bb{\frac{1}{d^{\frac{1}{4}}}}$. This requirement is similar in nature to contemporary work on Sparse PCA support recovery such as~\cite{meinshausen2006high, amini2008high, bresler2018sparse} where the leading eigenvector is assumed to have entries of the order $\Omega\bb{\frac{1}{\sqrt{s}}}$.
    % \rd We believe that this is an artifact of our moment-based analysis and can be relaxed with more sophisticated concentration inequalities. \bk
    %This is a much weaker assumption than that followed in contemporary work on Sparse PCA support recovery such as~\cite{meinshausen2006high, amini2008high, bresler2018sparse} where the leading eigenvector is assumed to have entries of the order $\Omega\bb{\frac{1}{\sqrt{s}}}$. However, we note that the results developed in these works stand valid under much smaller sample sizes $n = O\bb{\log\bb{d}}$. 
     % \rd What are the other papers with $s^2/n$\bk? 
\end{remark}
\begin{remark}
Note that Algorithm~\ref{alg:cardinality_support} requires simple initialization vectors $w_{0}, y_{0} \sim \mathcal{N}\bb{0,I}$. In contrast, the block stochastic power method-based algorithm presented in ~\cite{pmlr-v37-yangd15} provides local convergence guarantees (see Theorem 1) requiring a block size of $O\bb{s\log\bb{d}}$. They provide an initialization procedure, but the theoretical guarantees to achieve such an initialization require block size $\Omega\bb{d}$. \cite{yuan2011truncated} also require a close enough initialization. In the particular setting of a single-spiked covariance model, they require $|u_{0}^{T}v_{1}| = \Omega\bb{1}$. In comparison for Algorithm~\ref{alg:cardinality_support}, it suffices to have $|u_{0}^{T}v_{1}| \geq \frac{\delta}{\sqrt{e}}$ with probability at least $1-\delta$, using standard gaussian anti-concentration results (see Lemma~\ref{lemma:gaussian_anti_concentration}).
\end{remark}

% \rd
% \begin{remark}
%     In~\cite{berthet2013complexity}, the authors propose a computational lower bound for performing the following hypothesis test: 
%     \bas{
%         H_{0} : X \sim \mathcal{N}\bb{0, \id}, \;\; H_{1} : X \sim \mathcal{N}\bb{0, \id + \theta v_{1}v_{1}^{T}}   
%     }
%     and show that no polytime algorithm can discriminate the two hypotheses for $\theta \leq c\frac{s^{2}\log\bb{d}}{n}$, where $c > 0$ is a constant. 
%     Our result in Theorem~\ref{theorem:convergence_cardinality_support} does not violate this lower bound, since Assumption~\ref{assumption:high_dimensions} requires a higher eigengap $\frac{\lambda_{1}}{\lambda_{2}} \geq \widetilde{\Omega}\bb{1}$ which can be distinguished with polytime algorithms~\cite{berthet2013complexity}.
% \end{remark}
% \bk

Proof of Theorems~\ref{theorem:convergence_cardinality_support} is provided in Appendix Section~\ref{appendix:proofs_of_main_results}. We now present two important building blocks required for the proof of Theorem~\ref{theorem:convergence_cardinality_support} in Sections~\ref{section:one_step_power} and \ref{section:entrywise_deviation_oja}.
%\section{Our Techniques}
% Before we prove Theorem~\ref{theorem:convergence_truncated_oja}, we We start by analyzing the performance of Algorithm \ref{alg:truncated_oja} given an estimated support set $\widehat{S}$. For any set $\sh \subseteq [d]$, we define $I_{\sh} \in \mathbb{R}^{d \times d}$ as
% \bas{
%     I_{\sh}\bb{i,j} = \begin{cases}
%         1 \text{, if } i=j \text{ and } i \in \sh, \\
%         0 \text{, otherwise}
%     \end{cases}
% }
